Query-Focused Video Summarization: Dataset, Evaluation, and A Memory Network Based Approach

Recent years have witnessed a resurgence of interest in video summarization. However, one of the main obstacles to the research on video summarization is the user subjectivity - users have various preferences over the summaries. The subjectiveness causes at least two problems. First, no single video summarizer fits all users unless it interacts with and adapts to the individual users. Second, it is very challenging to evaluate the performance of a video summarizer. To tackle the first problem, we explore the recently proposed query-focused video summarization which introduces user preferences in the form of text queries about the video into the summarization process. We propose a memory network parameterized sequential determinantal point process in order to attend the user query onto different video frames and shots. To address the second challenge, we contend that a good evaluation metric for video summarization should focus on the semantic information that humans can perceive rather than the visual features or temporal overlaps. To this end, we collect dense per-video-shot concept annotations, compile a new dataset, and suggest an efficient evaluation method defined upon the concept annotations. We conduct extensive experiments contrasting our video summarizer to existing ones and present detailed analyses about the dataset and the new evaluation method.

==> Evaluation.tex <==
\section{Experimental Setup}
\label{subsec:eval}
In this section, we propose a new evaluation metric and contrast it against other existing metrics.

==> oracle.tex <==
% !Tex root = 1990-supp.tex
\section{Generating Oracle Summaries}
\label{Oracle}
Supervised video summarization methods often learn from one summary per video, or in the case of query-focused summarization per query-video pair. On the other hand, for evaluation purposes, it is better to contrast a system summary against multiple references and report the average. Thus, we collected 3 user summaries per query-video pair to use for evaluation purposes. However, in order to train the model, we obtain \textit{oracle} summaries that have maximum overall agreement with all three reference summaries (per query-video pair). 

The algorithm~\cite{kulesza2012determinantal} starts with the set of common shots ($y^0$) in all three reference summaries. Next, at each iteration, it greedily includes the shot that returns the largest marginal gain $G(i)$,
\begin{align}
\centering
G(i) = \sum_u \text{F1-score}(y^0\cup i,y_u) - \sum_u \text{F1-score}(y^0,y_u) 
\end{align}
where $u$ iterates over the user summaries (in our case, $u \in \{1,2,3\}$) and F1-score is obtained from our proposed evaluation metric. Table 1 in the main text shows the correlation between the obtained oracle summaries and user summaries, showing the oracle summary has very high agreement with all the user summaries.



==> query.tex <==
% !Tex root = 1990-supp.tex
\section{Constructing Queries}
\label{Queries}

In this section, we thoroughly describe the process of generating the queries from dense concept annotations. While users often input free text to query videos through search engines, we simulate the real scenarios and construct the queries using the dense concept annotations we have collected (cf.\ Section 3.2 in the main text) to ease benchmarking different algorithms. 
 
By processing the dense user annotation data, we extract various statistics that enable us to have the queries covering a wide range of varieties. Initially, a concept is assumed present in the video if it appears in at least $T$ shots. This is to filter the present noise in annotations acquired from AMT workers and to make sure the concepts really appear together (to steer clear of the pairs that are tagged together as a result of noise or bias). 

As described in the main text, when a user enters a query $q$ (for instance, on a video search engine), which is usually more than one word, we have four distinct scenarios; i) all the concepts in the query appear in the same video shots together, ii) all concepts appear in the video, but never jointly in a single shot, iii) only one of the concepts constituting the query appears in the some shots of the video, and iv) none of the concepts in the query are present in the video (1 such query). A robust video summarizer, must be able to maintain good performance under any of the scenarios. Therefore, by including enough samples of all the scenarios, we build a comprehensive and diverse dataset.

For the scenario i, we create a list of pairs that appear together in the same shots and sort it in descending order. There are two approaches to select concept pairs from this list: 1) to employ a random selection process where the probability of selecting a pair from the list is proportional to the number of times the pair appeared together in the video (this gives higher chance to the concepts that tend to happen together in the video while not completely crossing out the concepts that are not dominant in the video), and 2) to pick few top concept pairs. We opt to use the random selection process to better generalize the dataset and remove bias.

For the scenario ii, we are interested in concept pairs that are present in the video but not in the same shots, e.g., concept pairs such as \textsc{Car} and \textsc{Room} that are unlikely to appear in the same shots of the video. To this end, for each pair we compute their harmonic mean of frequencies:
\begin{equation}
	score(f_{c_1},f_{c_2}) = \frac{f_{c_1} \times f_{c_2}}{f_{c_1} + f_{c_2}}
\end{equation}
where $f_{c_1}$ and $f_{c_2}$ are the frequencies of concepts $c_1$ and $c_2$, respectively. This formulation has two interesting features that make it useful in this regard; 1) the resulting combination of numbers fed to it is always smaller than the smallest entry, 2) it is maximized when both inputs are large and identical. By computing the harmonic mean of frequencies for all the pairs in the list and sorting it in descending order, the concept pairs that have high frequencies for both concepts constituting the query are ranked higher. At this point, we employ the same random selection process to randomly choose pairs from this list.

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{./Caption_vs_tags2}
	\caption{\small{Comparing semantic information in our dense tags vs captions provided by~\cite{yeung2014videoset}. The figure illustrates that the caption is targeting limited information about the scene, while the dense annotations are able to better explain the characteristics of the scene.}}
	\label{fig:captionvstags}
\end{figure*}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{./Summary_comparison2}
	\caption{\small{This figure compares two user summaries (generated by the same user) for two different queries. Both summaries contain shared segments, that are assumed important in the context of the video, while they disagree on the query-relevant segments.}}
	\label{fig:sumcom}
\end{figure*}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{ROUGEvsIOU_Chng}
	\caption{\small{Studying the effect of randomly \textit{replacing} some video shots in the user summary on the performance. The evaluation by ROUGE-SU4~\cite{lin2004rouge} is included for reference.}}
	\label{fig:ROUGEvsIOU}
\end{figure*}

For the third scenario, we concentrate on pairs that only one concept constituting the query is present in the video, e.g., if there is no \textsc{Car} present in the entire video while there exists shots with \textsc{Computer} appearing in them, the pair \textsc{Car} and \textsc{Computer} is a candidate for this scenario. To make sure that the constructed dataset is comprehensive and benefits from the versatile dictionary, we first exclude the concepts that were used in the first two scenarios, we put the rest in a list and use their frequencies to randomly sample from them.

For the last scenario, where neither of concepts in pairs must be present in the video, we simply use the concepts that never appear in the video.

For scenarios i, ii, and iii, we select 15 queries. For scenario iv, we only choose one query; summarizing based on any such query consisting of concepts that are not present in the entire video must result in about the same summary. In other terms, when a user wants the model to summarize the video based on a query consisting of non-present concepts, the summarizer must only return \textit{contextually} important segments of the video, that is essentially what a conventional generic video summarization approach (as opposed to query-dependent approaches) generates.

Figure~\ref{fig:sumcom} shows that queries play a major role in the summaries that users generate. For a particular video, the same user has selected summaries that have both common (green margin) and uncommon (orange margin) segments.

==> rougevsiou.tex <==
% !Tex root = 1990-supp.tex
\section{Evaluation Metric Behavior}
\label{IOUvsROUGE}

As described in Section 5.2 of the main text, we studied the effect of randomly \textbf{removing} some video shots from the user summary on our proposed metric, observing that our metric has a linear drop in recall. Due to the fact that captions only capture limited information about the scene (cf.\ Figure~\ref{fig:captionvstags}), repeating the same experiment and evaluating with ROUGE-SU4 on captions provided by~\cite{yeung2014videoset}, recall showed a non-linear drop. As a side experiment, figure~\ref{fig:ROUGEvsIOU} illustrates the effect of randomly \textbf{replacing} some video shots in the user summary, studying the effect of noise on performance. Here we are swapping some shots with others that might be very similar or different to the original shots. For reference, we include the ROUGE-SU4 metric in our experiments as well.


